Accelerating Reductions Using Graph Neural Networks and a New Concurrent Local Search for the Maximum Weight Independent Set Problem

The Maximum Weight Independent Set problem is a fundamental NP-hard problem in combinatorial optimization with several real-world applications. Given an undirected vertex-weighted graph, the problem is to find a subset of the vertices with the highest possible weight under the constraint that no two vertices in the set can share an edge. An important part of solving this problem in both theory and practice is data reduction rules, which several state-of-the-art algorithms rely on. However, the most complicated rules are often not used in applications since the time needed to check them exhaustively becomes infeasible. In this work, we introduce three main results. First, we introduce several new data reduction rules and evaluate their effectiveness on real-world data. Second, we use a machine learning screening algorithm to speed up the reduction phase, thereby enabling more complicated rules to be applied. Our screening algorithm consults a Graph Neural Network oracle to decide if the probability of successfully reducing the graph is sufficiently large. For this task, we provide a dataset of labeled vertices for use in supervised learning. We also present the first results for this dataset using established Graph Neural Network architectures. Third, we present a new concurrent metaheuristic called Concurrent Difference-Core Heuristic. On the reduced instances, we use our new metaheuristic combined with iterated local search, called CHILS (Concurrent Hybrid Iterated Local Search). For this iterated local search, we provide a new implementation specifically designed to handle large graphs of varying densities. CHILS outperforms the current state-of-the-art on all commonly used benchmark instances, especially the largest ones.

==> data/datatool/baseTimePerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1.0146
0.146341463414634,1.0344
0.158536585365854,1.0395
0.170731707317073,1.0408
0.182926829268293,1.1074
0.195121951219512,1.2001
0.207317073170732,1.252
0.219512195121951,1.5549
0.231707317073171,1.7063
0.24390243902439,1.9803
0.25609756097561,1.9932
0.268292682926829,2.0902
0.280487804878049,2.3538
0.292682926829268,2.7177
0.304878048780488,3.672
0.317073170731707,3.821
0.329268292682927,3.9831
0.341463414634146,4.0128
0.353658536585366,4.0808
0.365853658536585,4.2903
0.378048780487805,4.3043
0.390243902439024,4.3065
0.402439024390244,4.6186
0.414634146341463,4.7731
0.426829268292683,5.2851
0.439024390243902,5.7899
0.451219512195122,7.7294
0.463414634146341,7.9804
0.475609756097561,8.3396
0.487804878048781,8.4286
0.5,9.2169
0.51219512195122,11.6232
0.524390243902439,23.8732
0.536585365853659,26.7588
0.548780487804878,27.0066
0.560975609756098,38.3013
0.573170731707317,47.6157
0.585365853658537,58.6349
0.597560975609756,69.7881
0.609756097560976,86.252
0.621951219512195,100
0.634146341463415,140.0871
0.646341463414634,140.1226
0.658536585365854,187.6477
0.670731707317073,207.3548
0.682926829268293,275.6272
0.695121951219512,359.8886
0.707317073170732,361.0528
0.719512195121951,391.9668
0.731707317073171,408.8221
0.74390243902439,483.0884
0.75609756097561,1142.8343
0.768292682926829,2784.8344
0.780487804878049,2844.9217
0.792682926829268,3031.3139
0.804878048780488,3053.173
0.817073170731707,3411.2386
0.829268292682927,4832.6536
0.841463414634146,4839.2517
0.853658536585366,4857.0318
0.865853658536585,6342.8897
0.878048780487805,6410.3838
0.890243902439024,6519.7902
0.902439024390244,6768.3741
0.914634146341463,7425.0535
0.926829268292683,12161.061
0.939024390243902,14302.3329
0.951219512195122,17231.0828
0.963414634146341,19814.6221
0.975609756097561,20097.2829
0.98780487804878,33120.0203
1,3599460100


==> data/datatool/baseWeightPerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1
0.146341463414634,1
0.158536585365854,1
0.170731707317073,1
0.182926829268293,1
0.195121951219512,1
0.207317073170732,1
0.219512195121951,1
0.231707317073171,1
0.24390243902439,1
0.25609756097561,1
0.268292682926829,1
0.280487804878049,1
0.292682926829268,1
0.304878048780488,1
0.317073170731707,1
0.329268292682927,1
0.341463414634146,1
0.353658536585366,1
0.365853658536585,1
0.378048780487805,1
0.390243902439024,1
0.402439024390244,1
0.414634146341463,1
0.426829268292683,1
0.439024390243902,1
0.451219512195122,1
0.463414634146341,1
0.475609756097561,1
0.487804878048781,1
0.5,1
0.51219512195122,1
0.524390243902439,1
0.536585365853659,1
0.548780487804878,1
0.560975609756098,1
0.573170731707317,1
0.585365853658537,1
0.597560975609756,1
0.609756097560976,1
0.621951219512195,1
0.634146341463415,1
0.646341463414634,1
0.658536585365854,1
0.670731707317073,1
0.682926829268293,1
0.695121951219512,1
0.707317073170732,1
0.719512195121951,1
0.731707317073171,1
0.74390243902439,1
0.75609756097561,1
0.768292682926829,1
0.780487804878049,0.9999
0.792682926829268,0.9999
0.804878048780488,0.9999
0.817073170731707,0.9999
0.829268292682927,0.9999
0.841463414634146,0.9999
0.853658536585366,0.9999
0.865853658536585,0.9999
0.878048780487805,0.9999
0.890243902439024,0.9999
0.902439024390244,0.9999
0.914634146341463,0.9998
0.926829268292683,0.9998
0.939024390243902,0.9997
0.951219512195122,0.9997
0.963414634146341,0.9996
0.975609756097561,0.9992
0.98780487804878,0.9988
1,0.9849


==> data/datatool/best_vr_baseWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,0.9998
0.166666666666667,0.9998
0.194444444444444,0.9996
0.222222222222222,0.9993
0.25,0.9989
0.277777777777778,0.9989
0.305555555555556,0.9987
0.333333333333333,0.9987
0.361111111111111,0.998
0.388888888888889,0.9978
0.416666666666667,0.9974
0.444444444444444,0.9973
0.472222222222222,0.9971
0.5,0.997
0.527777777777778,0.9964
0.555555555555556,0.9964
0.583333333333333,0.9963
0.611111111111111,0.9962
0.638888888888889,0.9961
0.666666666666667,0.996
0.694444444444444,0.996
0.722222222222222,0.9959
0.75,0.9958
0.777777777777778,0.9956
0.805555555555556,0.9953
0.833333333333333,0.9952
0.861111111111111,0.9951
0.888888888888889,0.995
0.916666666666667,0.9923
0.944444444444444,0.9917
0.972222222222222,0.99
1,0.9856


==> data/datatool/best_vr_chilsColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,0.9999
0.194444444444444,0.9999
0.222222222222222,0.9998
0.25,0.9998
0.277777777777778,0.9998
0.305555555555556,0.9997
0.333333333333333,0.9997
0.361111111111111,0.9993
0.388888888888889,0.9993
0.416666666666667,0.9992
0.444444444444444,0.9992
0.472222222222222,0.9992
0.5,0.999
0.527777777777778,0.9988
0.555555555555556,0.9986
0.583333333333333,0.9985
0.611111111111111,0.9984
0.638888888888889,0.998
0.666666666666667,0.998
0.694444444444444,0.9978
0.722222222222222,0.9977
0.75,0.9975
0.777777777777778,0.9974
0.805555555555556,0.9973
0.833333333333333,0.9972
0.861111111111111,0.9972
0.888888888888889,0.9971
0.916666666666667,0.997
0.944444444444444,0.9966
0.972222222222222,0.9966
1,0.9966


==> data/datatool/best_vr_chilsParWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,1
0.388888888888889,1
0.416666666666667,1
0.444444444444444,1
0.472222222222222,1
0.5,1
0.527777777777778,1
0.555555555555556,1
0.583333333333333,1
0.611111111111111,1
0.638888888888889,1
0.666666666666667,1
0.694444444444444,1
0.722222222222222,1
0.75,1
0.777777777777778,1
0.805555555555556,1
0.833333333333333,1
0.861111111111111,1
0.888888888888889,1
0.916666666666667,1
0.944444444444444,0.9998
0.972222222222222,0.9998
1,0.9992


==> data/datatool/best_vr_chilsRedWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,0.9999
0.277777777777778,0.9998
0.305555555555556,0.9997
0.333333333333333,0.9995
0.361111111111111,0.9993
0.388888888888889,0.9993
0.416666666666667,0.9988
0.444444444444444,0.9984
0.472222222222222,0.9973
0.5,0.9968
0.527777777777778,0.9958
0.555555555555556,0.9934
0.583333333333333,0.9924
0.611111111111111,0.9907
0.638888888888889,0.9901
0.666666666666667,0.9897
0.694444444444444,0.9888
0.722222222222222,0.9887
0.75,0.9878
0.777777777777778,0.9876
0.805555555555556,0.9865
0.833333333333333,0.9862
0.861111111111111,0.9861
0.888888888888889,0.9861
0.916666666666667,0.9844
0.944444444444444,0.9832
0.972222222222222,0.9813
1,0.9811


==> data/datatool/best_vr_chilsWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,0.9997
0.25,0.9996
0.277777777777778,0.9995
0.305555555555556,0.9993
0.333333333333333,0.9993
0.361111111111111,0.9993
0.388888888888889,0.9992
0.416666666666667,0.9992
0.444444444444444,0.9989
0.472222222222222,0.9989
0.5,0.9987
0.527777777777778,0.9987
0.555555555555556,0.9986
0.583333333333333,0.9985
0.611111111111111,0.9984
0.638888888888889,0.9984
0.666666666666667,0.9984
0.694444444444444,0.9982
0.722222222222222,0.9982
0.75,0.998
0.777777777777778,0.9979
0.805555555555556,0.9978
0.833333333333333,0.9978
0.861111111111111,0.9978
0.888888888888889,0.9976
0.916666666666667,0.9976
0.944444444444444,0.9972
0.972222222222222,0.9971
1,0.997


==> data/datatool/best_vr_ilpWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,0.999
0.333333333333333,0.999
0.361111111111111,0.999
0.388888888888889,0.999
0.416666666666667,0.998
0.444444444444444,0.996
0.472222222222222,0.995
0.5,0.994
0.527777777777778,0.992
0.555555555555556,0.991
0.583333333333333,0.991
0.611111111111111,0.989
0.638888888888889,0.989
0.666666666666667,0.989
0.694444444444444,0.988
0.722222222222222,0.988
0.75,0.987
0.777777777777778,0.987
0.805555555555556,0.986
0.833333333333333,0.986
0.861111111111111,0.986
0.888888888888889,0.986
0.916666666666667,0.984
0.944444444444444,0.983
0.972222222222222,0.953
1,0.914


==> data/datatool/best_vr_metamisColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,0.9998
0.25,0.9998
0.277777777777778,0.9996
0.305555555555556,0.9975
0.333333333333333,0.9971
0.361111111111111,0.997
0.388888888888889,0.9955
0.416666666666667,0.9953
0.444444444444444,0.9947
0.472222222222222,0.9931
0.5,0.9915
0.527777777777778,0.9907
0.555555555555556,0.9874
0.583333333333333,0.985
0.611111111111111,0.9834
0.638888888888889,0.9833
0.666666666666667,0.9827
0.694444444444444,0.9823
0.722222222222222,0.982
0.75,0.9808
0.777777777777778,0.9801
0.805555555555556,0.9792
0.833333333333333,0.9791
0.861111111111111,0.9784
0.888888888888889,0.9777
0.916666666666667,0.9773
0.944444444444444,0.9773
0.972222222222222,0.9766
1,0.9765


==> data/datatool/best_vr_metamisWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,0.9998
0.222222222222222,0.9997
0.25,0.9996
0.277777777777778,0.9992
0.305555555555556,0.9991
0.333333333333333,0.9991
0.361111111111111,0.999
0.388888888888889,0.9989
0.416666666666667,0.9988
0.444444444444444,0.9986
0.472222222222222,0.9985
0.5,0.9984
0.527777777777778,0.9982
0.555555555555556,0.9981
0.583333333333333,0.9981
0.611111111111111,0.9972
0.638888888888889,0.9971
0.666666666666667,0.9969
0.694444444444444,0.9969
0.722222222222222,0.9968
0.75,0.9966
0.777777777777778,0.9963
0.805555555555556,0.9963
0.833333333333333,0.9962
0.861111111111111,0.9959
0.888888888888889,0.9957
0.916666666666667,0.9957
0.944444444444444,0.9956
0.972222222222222,0.995
1,0.9949


==> data/datatool/chilsTimePerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1.007
0.0853658536585366,1.0088
0.0975609756097561,1.0344
0.109756097560976,1.0357
0.121951219512195,1.124
0.134146341463415,1.125
0.146341463414634,1.2
0.158536585365854,1.2043
0.170731707317073,1.2831
0.182926829268293,1.3075
0.195121951219512,1.597
0.207317073170732,1.8197
0.219512195121951,1.9383
0.231707317073171,1.9479
0.24390243902439,2
0.25609756097561,2.0345
0.268292682926829,2.1071
0.280487804878049,2.358
0.292682926829268,2.7022
0.304878048780488,3.821
0.317073170731707,3.948
0.329268292682927,4.0203
0.341463414634146,4.2426
0.353658536585366,4.3492
0.365853658536585,4.5218
0.378048780487805,4.5287
0.390243902439024,4.6896
0.402439024390244,4.7081
0.414634146341463,5.3572
0.426829268292683,5.7471
0.439024390243902,7.7852
0.451219512195122,8.3872
0.463414634146341,8.4242
0.475609756097561,9.3531
0.487804878048781,11.2251
0.5,16.0003
0.51219512195122,28.2932
0.524390243902439,29.1612
0.536585365853659,54.2471
0.548780487804878,66.6776
0.560975609756098,69.4374
0.573170731707317,90.135
0.585365853658537,100
0.597560975609756,140.0871
0.609756097560976,668.0685
0.621951219512195,838.2224
0.634146341463415,2037.5317
0.646341463414634,2206.3504
0.658536585365854,2398.8113
0.670731707317073,2985.0277
0.682926829268293,2996.1564
0.695121951219512,3129.985
0.707317073170732,3319.5649
0.719512195121951,3849.9543
0.731707317073171,4449.5716
0.74390243902439,4515.7792
0.75609756097561,4764.0345
0.768292682926829,4808.1335
0.780487804878049,4953.4805
0.792682926829268,4958.914
0.804878048780488,6089.0432
0.817073170731707,6564.6506
0.829268292682927,6748.746
0.841463414634146,6906.9507
0.853658536585366,7148.3344
0.865853658536585,8085.2005
0.878048780487805,8133.3506
0.890243902439024,8443.3525
0.902439024390244,10190.4008
0.914634146341463,10271.767
0.926829268292683,11984.8943
0.939024390243902,12466.1754
0.951219512195122,15348.947
0.963414634146341,20014.9087
0.975609756097561,23951.0924
0.98780487804878,30017.4424
1,3562854400


==> data/datatool/chilsWeightPerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1
0.146341463414634,1
0.158536585365854,1
0.170731707317073,1
0.182926829268293,1
0.195121951219512,1
0.207317073170732,1
0.219512195121951,1
0.231707317073171,1
0.24390243902439,1
0.25609756097561,1
0.268292682926829,1
0.280487804878049,1
0.292682926829268,1
0.304878048780488,1
0.317073170731707,1
0.329268292682927,1
0.341463414634146,1
0.353658536585366,1
0.365853658536585,1
0.378048780487805,1
0.390243902439024,1
0.402439024390244,1
0.414634146341463,1
0.426829268292683,1
0.439024390243902,1
0.451219512195122,1
0.463414634146341,1
0.475609756097561,1
0.487804878048781,1
0.5,1
0.51219512195122,1
0.524390243902439,1
0.536585365853659,1
0.548780487804878,1
0.560975609756098,1
0.573170731707317,1
0.585365853658537,1
0.597560975609756,1
0.609756097560976,1
0.621951219512195,1
0.634146341463415,1
0.646341463414634,1
0.658536585365854,1
0.670731707317073,1
0.682926829268293,1
0.695121951219512,1
0.707317073170732,1
0.719512195121951,1
0.731707317073171,1
0.74390243902439,1
0.75609756097561,1
0.768292682926829,1
0.780487804878049,1
0.792682926829268,1
0.804878048780488,1
0.817073170731707,1
0.829268292682927,1
0.841463414634146,1
0.853658536585366,1
0.865853658536585,1
0.878048780487805,1
0.890243902439024,1
0.902439024390244,1
0.914634146341463,0.9999
0.926829268292683,0.9999
0.939024390243902,0.9999
0.951219512195122,0.9998
0.963414634146341,0.9996
0.975609756097561,0.9996
0.98780487804878,0.9988
1,0.9948


==> data/datatool/hilsTimePerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1
0.146341463414634,1
0.158536585365854,1
0.170731707317073,1
0.182926829268293,1
0.195121951219512,1
0.207317073170732,1
0.219512195121951,1
0.231707317073171,1
0.24390243902439,1.101
0.25609756097561,1.2648
0.268292682926829,1.2757
0.280487804878049,1.71
0.292682926829268,1.8077
0.304878048780488,1.8442
0.317073170731707,1.8744
0.329268292682927,2.2314
0.341463414634146,2.7281
0.353658536585366,3.0092
0.365853658536585,3.2595
0.378048780487805,3.3001
0.390243902439024,3.6363
0.402439024390244,4.5694
0.414634146341463,4.7743
0.426829268292683,5.0226
0.439024390243902,5.0394
0.451219512195122,8.7583
0.463414634146341,9.388
0.475609756097561,9.6371
0.487804878048781,9.8694
0.5,36.5331
0.51219512195122,37.9192
0.524390243902439,57.7834
0.536585365853659,77.5875
0.548780487804878,91.4925
0.560975609756098,92.1143
0.573170731707317,94.1622
0.585365853658537,152.4272
0.597560975609756,198.3273
0.609756097560976,303.1159
0.621951219512195,838.0894
0.634146341463415,3075.6603
0.646341463414634,4834.7599
0.658536585365854,4982.2723
0.670731707317073,6271.7129
0.682926829268293,6559.0179
0.695121951219512,6942.3179
0.707317073170732,7315.558
0.719512195121951,7430.2338
0.731707317073171,7597.9451
0.74390243902439,8693.7578
0.75609756097561,9085.7026
0.768292682926829,9170.5854
0.780487804878049,10516.6844
0.792682926829268,12838.6779
0.804878048780488,17287.997
0.817073170731707,18074.9556
0.829268292682927,20207.8925
0.841463414634146,25890.8704
0.853658536585366,28132.3191
0.865853658536585,28308.5751
0.878048780487805,36566.4882
0.890243902439024,52054.3261
0.902439024390244,63018.9364
0.914634146341463,64976.0843
0.926829268292683,83096.2935
0.939024390243902,92324.1797
0.951219512195122,111834.2177
0.963414634146341,186477.3801
0.975609756097561,205160.6634
0.98780487804878,242299.7202
1,488788.9852


==> data/datatool/hilsWeightPerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1
0.146341463414634,1
0.158536585365854,1
0.170731707317073,1
0.182926829268293,1
0.195121951219512,1
0.207317073170732,1
0.219512195121951,1
0.231707317073171,1
0.24390243902439,1
0.25609756097561,1
0.268292682926829,1
0.280487804878049,1
0.292682926829268,1
0.304878048780488,1
0.317073170731707,1
0.329268292682927,1
0.341463414634146,1
0.353658536585366,1
0.365853658536585,1
0.378048780487805,1
0.390243902439024,1
0.402439024390244,1
0.414634146341463,1
0.426829268292683,1
0.439024390243902,1
0.451219512195122,1
0.463414634146341,1
0.475609756097561,1
0.487804878048781,1
0.5,1
0.51219512195122,1
0.524390243902439,1
0.536585365853659,1
0.548780487804878,0.9999
0.560975609756098,0.9999
0.573170731707317,0.9999
0.585365853658537,0.9999
0.597560975609756,0.9999
0.609756097560976,0.9997
0.621951219512195,0.9997
0.634146341463415,0.9996
0.646341463414634,0.9996
0.658536585365854,0.9995
0.670731707317073,0.9994
0.682926829268293,0.9994
0.695121951219512,0.9993
0.707317073170732,0.9991
0.719512195121951,0.9989
0.731707317073171,0.9989
0.74390243902439,0.9989
0.75609756097561,0.9988
0.768292682926829,0.9987
0.780487804878049,0.9984
0.792682926829268,0.9983
0.804878048780488,0.9976
0.817073170731707,0.9975
0.829268292682927,0.9952
0.841463414634146,0.9946
0.853658536585366,0.9945
0.865853658536585,0.9944
0.878048780487805,0.9923
0.890243902439024,0.9882
0.902439024390244,0.9881
0.914634146341463,0.9856
0.926829268292683,0.9836
0.939024390243902,0.9835
0.951219512195122,0.9801
0.963414634146341,0.9771
0.975609756097561,0.9769
0.98780487804878,0.9745
1,0.9731


==> data/datatool/htwisTimePerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1
0.146341463414634,1
0.158536585365854,1
0.170731707317073,1
0.182926829268293,1
0.195121951219512,1
0.207317073170732,1
0.219512195121951,1
0.231707317073171,1
0.24390243902439,1
0.25609756097561,1
0.268292682926829,1
0.280487804878049,1
0.292682926829268,1
0.304878048780488,1
0.317073170731707,1
0.329268292682927,1
0.341463414634146,1
0.353658536585366,1
0.365853658536585,1
0.378048780487805,1
0.390243902439024,1
0.402439024390244,1
0.414634146341463,1
0.426829268292683,1
0.439024390243902,1
0.451219512195122,1
0.463414634146341,1
0.475609756097561,1
0.487804878048781,1
0.5,1
0.51219512195122,1
0.524390243902439,1
0.536585365853659,1
0.548780487804878,1
0.560975609756098,1.0245
0.573170731707317,1.0302
0.585365853658537,1.0611
0.597560975609756,1.1173
0.609756097560976,1.2777
0.621951219512195,1.4399
0.634146341463415,1.5272
0.646341463414634,1.6614
0.658536585365854,1.7033
0.670731707317073,2.01
0.682926829268293,2.0555
0.695121951219512,2.8599
0.707317073170732,3.2853
0.719512195121951,3.463
0.731707317073171,3.5049
0.74390243902439,3.6746
0.75609756097561,3.7357
0.768292682926829,4.3367
0.780487804878049,4.4912
0.792682926829268,5.3678
0.804878048780488,5.4229
0.817073170731707,5.757
0.829268292682927,6.5597
0.841463414634146,6.5918
0.853658536585366,6.7469
0.865853658536585,7.9845
0.878048780487805,8.7751
0.890243902439024,10.2776
0.902439024390244,13.2182
0.914634146341463,13.542
0.926829268292683,16.6578
0.939024390243902,19.075
0.951219512195122,41.7038
0.963414634146341,42.9881
0.975609756097561,86.9499
0.98780487804878,532
1,9219021


==> data/datatool/htwisWeightPerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,0.9999
0.0487804878048781,0.9999
0.0609756097560976,0.9999
0.0731707317073171,0.9999
0.0853658536585366,0.9999
0.0975609756097561,0.9998
0.109756097560976,0.9997
0.121951219512195,0.9997
0.134146341463415,0.9997
0.146341463414634,0.9996
0.158536585365854,0.9996
0.170731707317073,0.9996
0.182926829268293,0.9993
0.195121951219512,0.9992
0.207317073170732,0.9992
0.219512195121951,0.9992
0.231707317073171,0.9991
0.24390243902439,0.999
0.25609756097561,0.999
0.268292682926829,0.999
0.280487804878049,0.9989
0.292682926829268,0.9989
0.304878048780488,0.9988
0.317073170731707,0.9988
0.329268292682927,0.9988
0.341463414634146,0.9986
0.353658536585366,0.9984
0.365853658536585,0.9979
0.378048780487805,0.9972
0.390243902439024,0.9967
0.402439024390244,0.9955
0.414634146341463,0.9953
0.426829268292683,0.995
0.439024390243902,0.9944
0.451219512195122,0.9942
0.463414634146341,0.9937
0.475609756097561,0.9923
0.487804878048781,0.9917
0.5,0.9913
0.51219512195122,0.9906
0.524390243902439,0.9903
0.536585365853659,0.9901
0.548780487804878,0.9898
0.560975609756098,0.9889
0.573170731707317,0.9871
0.585365853658537,0.9869
0.597560975609756,0.9857
0.609756097560976,0.9853
0.621951219512195,0.9848
0.634146341463415,0.9842
0.646341463414634,0.9836
0.658536585365854,0.9834
0.670731707317073,0.9832
0.682926829268293,0.9824
0.695121951219512,0.9823
0.707317073170732,0.982
0.719512195121951,0.9817
0.731707317073171,0.9812
0.74390243902439,0.9796
0.75609756097561,0.9794
0.768292682926829,0.979
0.780487804878049,0.979
0.792682926829268,0.9787
0.804878048780488,0.9741
0.817073170731707,0.9741
0.829268292682927,0.9721
0.841463414634146,0.9717
0.853658536585366,0.9705
0.865853658536585,0.9705
0.878048780487805,0.967
0.890243902439024,0.9623
0.902439024390244,0.9559
0.914634146341463,0.9547
0.926829268292683,0.9497
0.939024390243902,0.9483
0.951219512195122,0.9434
0.963414634146341,0.9401
0.975609756097561,0.9386
0.98780487804878,0.9244
1,0.8924


==> data/datatool/kernel_data/kernel_baseTimePerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1.0705
0.193548387096774,1.1101
0.225806451612903,1.1939
0.258064516129032,1.3456
0.290322580645161,1.5491
0.32258064516129,1.8522
0.354838709677419,2.7074
0.387096774193548,2.7514
0.419354838709677,4.0485
0.451612903225806,4.8437
0.483870967741936,5.4002
0.516129032258065,6.415
0.548387096774194,6.6164
0.580645161290323,6.8584
0.612903225806452,7.1571
0.645161290322581,9.487
0.67741935483871,12.0064
0.709677419354839,12.3853
0.741935483870968,15.5896
0.774193548387097,23.0694
0.806451612903226,23.7901
0.838709677419355,24.8766
0.870967741935484,52.9514
0.903225806451613,139.9037
0.935483870967742,144.394
0.967741935483871,184.3548
1,947.4643


==> data/datatool/kernel_data/kernel_baseWeightPerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1
0.193548387096774,1
0.225806451612903,1
0.258064516129032,1
0.290322580645161,1
0.32258064516129,1
0.354838709677419,1
0.387096774193548,1
0.419354838709677,1
0.451612903225806,1
0.483870967741936,1
0.516129032258065,1
0.548387096774194,1
0.580645161290323,1
0.612903225806452,1
0.645161290322581,1
0.67741935483871,1
0.709677419354839,1
0.741935483870968,1
0.774193548387097,1
0.806451612903226,1
0.838709677419355,0.9998
0.870967741935484,0.9995
0.903225806451613,0.9992
0.935483870967742,0.9973
0.967741935483871,0.9952
1,0.995


==> data/datatool/kernel_data/kernel_chilsTimePerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1.3034
0.161290322580645,1.3303
0.193548387096774,2.564
0.225806451612903,2.653
0.258064516129032,2.7514
0.290322580645161,4.064
0.32258064516129,4.8165
0.354838709677419,5.3781
0.387096774193548,6.2542
0.419354838709677,6.373
0.451612903225806,6.4234
0.483870967741936,7.2264
0.516129032258065,7.5896
0.548387096774194,9.7354
0.580645161290323,11.0353
0.612903225806452,11.6208
0.645161290322581,12.4551
0.67741935483871,13.2841
0.709677419354839,13.7294
0.741935483870968,20.9057
0.774193548387097,22.7543
0.806451612903226,22.9758
0.838709677419355,51.9097
0.870967741935484,130.0692
0.903225806451613,131.9786
0.935483870967742,197.8615
0.967741935483871,1517.8384
1,8992.3601


==> data/datatool/kernel_data/kernel_chilsWeightPerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1
0.193548387096774,1
0.225806451612903,1
0.258064516129032,1
0.290322580645161,1
0.32258064516129,1
0.354838709677419,1
0.387096774193548,1
0.419354838709677,1
0.451612903225806,1
0.483870967741936,1
0.516129032258065,1
0.548387096774194,1
0.580645161290323,1
0.612903225806452,1
0.645161290322581,1
0.67741935483871,1
0.709677419354839,1
0.741935483870968,1
0.774193548387097,1
0.806451612903226,1
0.838709677419355,1
0.870967741935484,1
0.903225806451613,1
0.935483870967742,1
0.967741935483871,1
1,1


==> data/datatool/kernel_data/kernel_hilsTimePerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1
0.193548387096774,1
0.225806451612903,1
0.258064516129032,1
0.290322580645161,1
0.32258064516129,1
0.354838709677419,1
0.387096774193548,1
0.419354838709677,1.5151
0.451612903225806,1.6311
0.483870967741936,1.6753
0.516129032258065,2.0587
0.548387096774194,2.1569
0.580645161290323,2.1783
0.612903225806452,2.5167
0.645161290322581,2.6319
0.67741935483871,7.3586
0.709677419354839,7.8571
0.741935483870968,8.8613
0.774193548387097,13.4435
0.806451612903226,142.606
0.838709677419355,239.2379
0.870967741935484,262.3086
0.903225806451613,451.0259
0.935483870967742,7640.9529
0.967741935483871,13124.5795
1,50155.8066


==> data/datatool/kernel_data/kernel_hilsWeightPerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1
0.193548387096774,1
0.225806451612903,1
0.258064516129032,1
0.290322580645161,1
0.32258064516129,1
0.354838709677419,1
0.387096774193548,1
0.419354838709677,1
0.451612903225806,1
0.483870967741936,1
0.516129032258065,1
0.548387096774194,1
0.580645161290323,1
0.612903225806452,1
0.645161290322581,1
0.67741935483871,1
0.709677419354839,1
0.741935483870968,1
0.774193548387097,1
0.806451612903226,0.9993
0.838709677419355,0.9987
0.870967741935484,0.998
0.903225806451613,0.9971
0.935483870967742,0.9958
0.967741935483871,0.9943
1,0.9925


==> data/datatool/kernel_data/kernel_htwisTimePerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1
0.193548387096774,1
0.225806451612903,1
0.258064516129032,1
0.290322580645161,1
0.32258064516129,1.2134
0.354838709677419,1.6207
0.387096774193548,1.6416
0.419354838709677,1.7468
0.451612903225806,2.568
0.483870967741936,2.7527
0.516129032258065,2.9058
0.548387096774194,3.9558
0.580645161290323,4.4284
0.612903225806452,4.6816
0.645161290322581,5.7347
0.67741935483871,6.6744
0.709677419354839,7.1155
0.741935483870968,8.2925
0.774193548387097,9.4612
0.806451612903226,10.6377
0.838709677419355,16.8333
0.870967741935484,17.8887
0.903225806451613,34.1613
0.935483870967742,41.4233
0.967741935483871,43.0851
1,190.1503


==> data/datatool/kernel_data/kernel_htwisWeightPerf.tex <==
fraction,perf
0,1
0.032258064516129,0.9974
0.0645161290322581,0.996
0.0967741935483871,0.9914
0.129032258064516,0.9904
0.161290322580645,0.985
0.193548387096774,0.982
0.225806451612903,0.9759
0.258064516129032,0.9755
0.290322580645161,0.9703
0.32258064516129,0.9667
0.354838709677419,0.9359
0.387096774193548,0.9288
0.419354838709677,0.9256
0.451612903225806,0.9255
0.483870967741936,0.9243
0.516129032258065,0.9194
0.548387096774194,0.9178
0.580645161290323,0.9172
0.612903225806452,0.9168
0.645161290322581,0.9128
0.67741935483871,0.8871
0.709677419354839,0.883
0.741935483870968,0.8757
0.774193548387097,0.8751
0.806451612903226,0.8645
0.838709677419355,0.8632
0.870967741935484,0.8611
0.903225806451613,0.859
0.935483870967742,0.8574
0.967741935483871,0.8559
1,0.8516


==> data/datatool/kernel_data/kernel_mmwisTimePerf.tex <==
fraction,perf
0,5.4979
0.032258064516129,40.0277
0.0645161290322581,52.36
0.0967741935483871,120.8494
0.129032258064516,145.2973
0.161290322580645,165.2708
0.193548387096774,208.8077
0.225806451612903,229.7926
0.258064516129032,313.4175
0.290322580645161,954.8843
0.32258064516129,1600.5222
0.354838709677419,1698.5017
0.387096774193548,2390.646
0.419354838709677,2409.6416
0.451612903225806,3154.1582
0.483870967741936,3507.402
0.516129032258065,4357.0171
0.548387096774194,5184.281
0.580645161290323,6060.6875
0.612903225806452,7456.2485
0.645161290322581,8151.3438
0.67741935483871,9973.4129
0.709677419354839,11861.4249
0.741935483870968,12701.291
0.774193548387097,15543.7062
0.806451612903226,24912.0887
0.838709677419355,29684.0486
0.870967741935484,34742.3032
0.903225806451613,65495.4545
0.935483870967742,65495.9979
0.967741935483871,82393.5923
1,563994.6483


==> data/datatool/kernel_data/kernel_mmwisWeightPerf.tex <==
fraction,perf
0,1
0.032258064516129,1
0.0645161290322581,1
0.0967741935483871,1
0.129032258064516,1
0.161290322580645,1
0.193548387096774,1
0.225806451612903,1
0.258064516129032,1
0.290322580645161,1
0.32258064516129,1
0.354838709677419,1
0.387096774193548,1
0.419354838709677,1
0.451612903225806,1
0.483870967741936,1
0.516129032258065,1
0.548387096774194,1
0.580645161290323,1
0.612903225806452,1
0.645161290322581,1
0.67741935483871,1
0.709677419354839,1
0.741935483870968,1
0.774193548387097,1
0.806451612903226,1
0.838709677419355,0.9999
0.870967741935484,0.9996
0.903225806451613,0.9996
0.935483870967742,0.9783
0.967741935483871,0.9632
1,0.918


==> data/datatool/mmwisTimePerf.tex <==
fraction,perf
0,1
0.0121951219512195,1.0183
0.024390243902439,1.451
0.0365853658536585,1.7848
0.0487804878048781,2.2814
0.0609756097560976,2.4763
0.0731707317073171,2.549
0.0853658536585366,2.6283
0.0975609756097561,2.6496
0.109756097560976,2.9044
0.121951219512195,3.1697
0.134146341463415,3.7297
0.146341463414634,3.7379
0.158536585365854,3.9958
0.170731707317073,4.0061
0.182926829268293,4.1285
0.195121951219512,4.1684
0.207317073170732,4.7053
0.219512195121951,4.8494
0.231707317073171,4.8548
0.24390243902439,4.9623
0.25609756097561,5.3642
0.268292682926829,5.621
0.280487804878049,5.7035
0.292682926829268,5.769
0.304878048780488,6.0737
0.317073170731707,7.3148
0.329268292682927,8.209
0.341463414634146,10.0882
0.353658536585366,11.622
0.365853658536585,14.2556
0.378048780487805,15.8073
0.390243902439024,18.2651
0.402439024390244,19.4657
0.414634146341463,22.924
0.426829268292683,25.5984
0.439024390243902,27.223
0.451219512195122,28.2889
0.463414634146341,35.1701
0.475609756097561,39.759
0.487804878048781,41.5645
0.5,45.6722
0.51219512195122,52.6795
0.524390243902439,57.965
0.536585365853659,58.4687
0.548780487804878,76.5339
0.560975609756098,81.6696
0.573170731707317,89.8264
0.585365853658537,93.1119
0.597560975609756,95.2922
0.609756097560976,95.4761
0.621951219512195,104.1128
0.634146341463415,113.2628
0.646341463414634,122.9776
0.658536585365854,126.3125
0.670731707317073,149.2861
0.682926829268293,164.2054
0.695121951219512,168.1201
0.707317073170732,170.0063
0.719512195121951,199.4473
0.731707317073171,217.2262
0.74390243902439,252.1851
0.75609756097561,294.6835
0.768292682926829,300.8589
0.780487804878049,344.5005
0.792682926829268,369.4989
0.804878048780488,422.2082
0.817073170731707,428.1908
0.829268292682927,463.84
0.841463414634146,684.0035
0.853658536585366,743.7777
0.865853658536585,972.0198
0.878048780487805,1880.88
0.890243902439024,2418.0645
0.902439024390244,2483.5262
0.914634146341463,3157.7919
0.926829268292683,4226.4125
0.939024390243902,6565.5081
0.951219512195122,11632.8133
0.963414634146341,25155.3486
0.975609756097561,53720.6558
0.98780487804878,83575.7885
1,1737390000


==> data/datatool/mmwisWeightPerf.tex <==
fraction,perf
0,1
0.0121951219512195,1
0.024390243902439,1
0.0365853658536585,1
0.0487804878048781,1
0.0609756097560976,1
0.0731707317073171,1
0.0853658536585366,1
0.0975609756097561,1
0.109756097560976,1
0.121951219512195,1
0.134146341463415,1
0.146341463414634,1
0.158536585365854,1
0.170731707317073,1
0.182926829268293,1
0.195121951219512,1
0.207317073170732,1
0.219512195121951,1
0.231707317073171,1
0.24390243902439,1
0.25609756097561,1
0.268292682926829,1
0.280487804878049,1
0.292682926829268,1
0.304878048780488,1
0.317073170731707,1
0.329268292682927,1
0.341463414634146,1
0.353658536585366,1
0.365853658536585,1
0.378048780487805,1
0.390243902439024,1
0.402439024390244,1
0.414634146341463,1
0.426829268292683,1
0.439024390243902,1
0.451219512195122,1
0.463414634146341,1
0.475609756097561,1
0.487804878048781,1
0.5,1
0.51219512195122,1
0.524390243902439,1
0.536585365853659,1
0.548780487804878,1
0.560975609756098,1
0.573170731707317,1
0.585365853658537,1
0.597560975609756,1
0.609756097560976,1
0.621951219512195,1
0.634146341463415,1
0.646341463414634,1
0.658536585365854,1
0.670731707317073,1
0.682926829268293,1
0.695121951219512,1
0.707317073170732,1
0.719512195121951,1
0.731707317073171,1
0.74390243902439,1
0.75609756097561,1
0.768292682926829,1
0.780487804878049,1
0.792682926829268,1
0.804878048780488,1
0.817073170731707,1
0.829268292682927,1
0.841463414634146,1
0.853658536585366,1
0.865853658536585,1
0.878048780487805,1
0.890243902439024,1
0.902439024390244,1
0.914634146341463,1
0.926829268292683,0.9999
0.939024390243902,0.9999
0.951219512195122,0.9998
0.963414634146341,0.9983
0.975609756097561,0.9941
0.98780487804878,0.9739
1,0.9658


==> data/datatool/vr10_baseWeightPerf.tex <==
fraction,perf
0,1.0005
0.0277777777777778,1.0004
0.0555555555555556,1.0002
0.0833333333333333,1.0002
0.111111111111111,1.0002
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,0.9999
0.305555555555556,0.9999
0.333333333333333,0.9999
0.361111111111111,0.9998
0.388888888888889,0.9997
0.416666666666667,0.9997
0.444444444444444,0.9997
0.472222222222222,0.9997
0.5,0.9996
0.527777777777778,0.9996
0.555555555555556,0.9996
0.583333333333333,0.9991
0.611111111111111,0.999
0.638888888888889,0.9989
0.666666666666667,0.9989
0.694444444444444,0.9988
0.722222222222222,0.9986
0.75,0.9985
0.777777777777778,0.9976
0.805555555555556,0.9968
0.833333333333333,0.9952
0.861111111111111,0.994
0.888888888888889,0.9934
0.916666666666667,0.9923
0.944444444444444,0.9898
0.972222222222222,0.9853
1,0.984


==> data/datatool/vr10_chilsColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,0.9999
0.194444444444444,0.9998
0.222222222222222,0.9998
0.25,0.9997
0.277777777777778,0.9997
0.305555555555556,0.9996
0.333333333333333,0.9993
0.361111111111111,0.9991
0.388888888888889,0.9985
0.416666666666667,0.9984
0.444444444444444,0.9983
0.472222222222222,0.9982
0.5,0.9978
0.527777777777778,0.9977
0.555555555555556,0.9973
0.583333333333333,0.9969
0.611111111111111,0.9968
0.638888888888889,0.9964
0.666666666666667,0.9963
0.694444444444444,0.9961
0.722222222222222,0.9958
0.75,0.9955
0.777777777777778,0.9954
0.805555555555556,0.9951
0.833333333333333,0.995
0.861111111111111,0.9949
0.888888888888889,0.9948
0.916666666666667,0.9944
0.944444444444444,0.9943
0.972222222222222,0.9938
1,0.9931


==> data/datatool/vr10_chilsWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,1
0.388888888888889,1
0.416666666666667,1
0.444444444444444,1
0.472222222222222,1
0.5,1
0.527777777777778,1
0.555555555555556,1
0.583333333333333,0.9999
0.611111111111111,0.9999
0.638888888888889,0.9998
0.666666666666667,0.9998
0.694444444444444,0.9997
0.722222222222222,0.9997
0.75,0.9996
0.777777777777778,0.9996
0.805555555555556,0.9996
0.833333333333333,0.9994
0.861111111111111,0.9992
0.888888888888889,0.9992
0.916666666666667,0.9986
0.944444444444444,0.998
0.972222222222222,0.9969
1,0.9952


==> data/datatool/vr10_ilpWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,0.9998
0.388888888888889,0.9995
0.416666666666667,0.9957
0.444444444444444,0.995
0.472222222222222,0.9948
0.5,0.9934
0.527777777777778,0.993
0.555555555555556,0.9921
0.583333333333333,0.9915
0.611111111111111,0.9899
0.638888888888889,0.9886
0.666666666666667,0.9875
0.694444444444444,0.9872
0.722222222222222,0.9866
0.75,0.9859
0.777777777777778,0.9855
0.805555555555556,0.9848
0.833333333333333,0.9814
0.861111111111111,0.9804
0.888888888888889,0.9455
0.916666666666667,0.9103
0.944444444444444,0.4165
0.972222222222222,0.4128
1,0.4086


==> data/datatool/vr10_metamisColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,0.9995
0.166666666666667,0.9995
0.194444444444444,0.9994
0.222222222222222,0.9994
0.25,0.9989
0.277777777777778,0.9985
0.305555555555556,0.9978
0.333333333333333,0.9978
0.361111111111111,0.9968
0.388888888888889,0.996
0.416666666666667,0.9945
0.444444444444444,0.9914
0.472222222222222,0.9907
0.5,0.9888
0.527777777777778,0.987
0.555555555555556,0.9825
0.583333333333333,0.9815
0.611111111111111,0.981
0.638888888888889,0.9805
0.666666666666667,0.9802
0.694444444444444,0.9797
0.722222222222222,0.9797
0.75,0.9796
0.777777777777778,0.9792
0.805555555555556,0.9791
0.833333333333333,0.9783
0.861111111111111,0.9771
0.888888888888889,0.9755
0.916666666666667,0.9755
0.944444444444444,0.9752
0.972222222222222,0.9752
1,0.9749


==> data/datatool/vr10_metamisWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,0.9999
0.333333333333333,0.9999
0.361111111111111,0.9998
0.388888888888889,0.9998
0.416666666666667,0.9998
0.444444444444444,0.9997
0.472222222222222,0.9997
0.5,0.9996
0.527777777777778,0.9996
0.555555555555556,0.9996
0.583333333333333,0.9995
0.611111111111111,0.9995
0.638888888888889,0.9995
0.666666666666667,0.9994
0.694444444444444,0.9993
0.722222222222222,0.9993
0.75,0.9992
0.777777777777778,0.9992
0.805555555555556,0.9991
0.833333333333333,0.9991
0.861111111111111,0.999
0.888888888888889,0.9986
0.916666666666667,0.9981
0.944444444444444,0.9975
0.972222222222222,0.9968
1,0.9947


==> data/datatool/vr50_baseWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,0.9998
0.166666666666667,0.9998
0.194444444444444,0.9996
0.222222222222222,0.9995
0.25,0.9995
0.277777777777778,0.9994
0.305555555555556,0.9993
0.333333333333333,0.9989
0.361111111111111,0.9989
0.388888888888889,0.9986
0.416666666666667,0.9986
0.444444444444444,0.9986
0.472222222222222,0.9984
0.5,0.9982
0.527777777777778,0.9981
0.555555555555556,0.9981
0.583333333333333,0.998
0.611111111111111,0.998
0.638888888888889,0.9979
0.666666666666667,0.9978
0.694444444444444,0.9976
0.722222222222222,0.9974
0.75,0.9974
0.777777777777778,0.9974
0.805555555555556,0.9971
0.833333333333333,0.9969
0.861111111111111,0.9957
0.888888888888889,0.9952
0.916666666666667,0.9931
0.944444444444444,0.9922
0.972222222222222,0.9902
1,0.9856


==> data/datatool/vr50_chilsColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,0.9999
0.333333333333333,0.9999
0.361111111111111,0.9999
0.388888888888889,0.9999
0.416666666666667,0.9998
0.444444444444444,0.9998
0.472222222222222,0.9993
0.5,0.9993
0.527777777777778,0.9992
0.555555555555556,0.9991
0.583333333333333,0.9991
0.611111111111111,0.9991
0.638888888888889,0.999
0.666666666666667,0.9987
0.694444444444444,0.9987
0.722222222222222,0.9985
0.75,0.9985
0.777777777777778,0.9984
0.805555555555556,0.9983
0.833333333333333,0.9983
0.861111111111111,0.9981
0.888888888888889,0.998
0.916666666666667,0.9978
0.944444444444444,0.9978
0.972222222222222,0.9973
1,0.9965


==> data/datatool/vr50_chilsWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,1
0.388888888888889,1
0.416666666666667,1
0.444444444444444,1
0.472222222222222,1
0.5,1
0.527777777777778,1
0.555555555555556,1
0.583333333333333,0.9999
0.611111111111111,0.9999
0.638888888888889,0.9999
0.666666666666667,0.9998
0.694444444444444,0.9998
0.722222222222222,0.9998
0.75,0.9997
0.777777777777778,0.9996
0.805555555555556,0.9996
0.833333333333333,0.9996
0.861111111111111,0.9992
0.888888888888889,0.9991
0.916666666666667,0.9987
0.944444444444444,0.9986
0.972222222222222,0.997
1,0.9968


==> data/datatool/vr50_ilpWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,0.9998
0.361111111111111,0.9996
0.388888888888889,0.9993
0.416666666666667,0.998
0.444444444444444,0.9966
0.472222222222222,0.9952
0.5,0.9949
0.527777777777778,0.993
0.555555555555556,0.9928
0.583333333333333,0.9917
0.611111111111111,0.9912
0.638888888888889,0.9894
0.666666666666667,0.9891
0.694444444444444,0.989
0.722222222222222,0.9886
0.75,0.9881
0.777777777777778,0.9879
0.805555555555556,0.9878
0.833333333333333,0.9875
0.861111111111111,0.9862
0.888888888888889,0.9861
0.916666666666667,0.9842
0.944444444444444,0.9839
0.972222222222222,0.9533
1,0.9119


==> data/datatool/vr50_metamisColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,0.9999
0.222222222222222,0.9998
0.25,0.9997
0.277777777777778,0.9996
0.305555555555556,0.9979
0.333333333333333,0.9975
0.361111111111111,0.9975
0.388888888888889,0.9965
0.416666666666667,0.9947
0.444444444444444,0.994
0.472222222222222,0.9925
0.5,0.9915
0.527777777777778,0.9901
0.555555555555556,0.9856
0.583333333333333,0.985
0.611111111111111,0.9838
0.638888888888889,0.983
0.666666666666667,0.9826
0.694444444444444,0.9819
0.722222222222222,0.9816
0.75,0.9809
0.777777777777778,0.9803
0.805555555555556,0.9801
0.833333333333333,0.9798
0.861111111111111,0.9788
0.888888888888889,0.9784
0.916666666666667,0.9781
0.944444444444444,0.9776
0.972222222222222,0.9774
1,0.9764


==> data/datatool/vr50_metamisWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,0.9998
0.277777777777778,0.9998
0.305555555555556,0.9998
0.333333333333333,0.9997
0.361111111111111,0.9996
0.388888888888889,0.9994
0.416666666666667,0.9993
0.444444444444444,0.9992
0.472222222222222,0.9992
0.5,0.999
0.527777777777778,0.999
0.555555555555556,0.9987
0.583333333333333,0.9985
0.611111111111111,0.9985
0.638888888888889,0.9985
0.666666666666667,0.9984
0.694444444444444,0.9984
0.722222222222222,0.9982
0.75,0.9981
0.777777777777778,0.9981
0.805555555555556,0.998
0.833333333333333,0.9976
0.861111111111111,0.9973
0.888888888888889,0.9972
0.916666666666667,0.9972
0.944444444444444,0.9971
0.972222222222222,0.9967
1,0.995


==> data/datatool/vr_baseWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,0.9998
0.166666666666667,0.9998
0.194444444444444,0.9997
0.222222222222222,0.9996
0.25,0.9995
0.277777777777778,0.9995
0.305555555555556,0.9994
0.333333333333333,0.9989
0.361111111111111,0.9989
0.388888888888889,0.9986
0.416666666666667,0.9986
0.444444444444444,0.9985
0.472222222222222,0.9985
0.5,0.9984
0.527777777777778,0.9983
0.555555555555556,0.9981
0.583333333333333,0.9981
0.611111111111111,0.998
0.638888888888889,0.998
0.666666666666667,0.9977
0.694444444444444,0.9977
0.722222222222222,0.9976
0.75,0.9975
0.777777777777778,0.9971
0.805555555555556,0.9969
0.833333333333333,0.9967
0.861111111111111,0.9957
0.888888888888889,0.9957
0.916666666666667,0.9934
0.944444444444444,0.992
0.972222222222222,0.99
1,0.9856


==> data/datatool/vr_chilsColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,1
0.388888888888889,1
0.416666666666667,0.9999
0.444444444444444,0.9999
0.472222222222222,0.9998
0.5,0.9998
0.527777777777778,0.9998
0.555555555555556,0.9998
0.583333333333333,0.9997
0.611111111111111,0.9997
0.638888888888889,0.9996
0.666666666666667,0.9995
0.694444444444444,0.9993
0.722222222222222,0.9993
0.75,0.9992
0.777777777777778,0.9992
0.805555555555556,0.9992
0.833333333333333,0.9988
0.861111111111111,0.9987
0.888888888888889,0.9986
0.916666666666667,0.9986
0.944444444444444,0.9985
0.972222222222222,0.9982
1,0.998


==> data/datatool/vr_chilsWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,1
0.388888888888889,1
0.416666666666667,1
0.444444444444444,1
0.472222222222222,1
0.5,1
0.527777777777778,1
0.555555555555556,1
0.583333333333333,1
0.611111111111111,1
0.638888888888889,0.9998
0.666666666666667,0.9997
0.694444444444444,0.9997
0.722222222222222,0.9996
0.75,0.9996
0.777777777777778,0.9996
0.805555555555556,0.9995
0.833333333333333,0.9992
0.861111111111111,0.9992
0.888888888888889,0.9991
0.916666666666667,0.999
0.944444444444444,0.9987
0.972222222222222,0.9975
1,0.9971


==> data/datatool/vr_ilpWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,1
0.277777777777778,1
0.305555555555556,1
0.333333333333333,1
0.361111111111111,1
0.388888888888889,0.999
0.416666666666667,0.998
0.444444444444444,0.997
0.472222222222222,0.995
0.5,0.995
0.527777777777778,0.993
0.555555555555556,0.993
0.583333333333333,0.992
0.611111111111111,0.992
0.638888888888889,0.99
0.666666666666667,0.99
0.694444444444444,0.989
0.722222222222222,0.989
0.75,0.989
0.777777777777778,0.988
0.805555555555556,0.988
0.833333333333333,0.988
0.861111111111111,0.988
0.888888888888889,0.987
0.916666666666667,0.985
0.944444444444444,0.985
0.972222222222222,0.953
1,0.914


==> data/datatool/vr_metamisColdWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,1
0.222222222222222,1
0.25,0.9998
0.277777777777778,0.9996
0.305555555555556,0.9982
0.333333333333333,0.9976
0.361111111111111,0.9974
0.388888888888889,0.9967
0.416666666666667,0.9953
0.444444444444444,0.9947
0.472222222222222,0.9933
0.5,0.9923
0.527777777777778,0.9915
0.555555555555556,0.9877
0.583333333333333,0.9858
0.611111111111111,0.9848
0.638888888888889,0.9844
0.666666666666667,0.9839
0.694444444444444,0.9834
0.722222222222222,0.9834
0.75,0.9823
0.777777777777778,0.9823
0.805555555555556,0.9815
0.833333333333333,0.9808
0.861111111111111,0.9803
0.888888888888889,0.9803
0.916666666666667,0.9798
0.944444444444444,0.9795
0.972222222222222,0.9786
1,0.978


==> data/datatool/vr_metamisWarmWeightPerf.tex <==
fraction,perf
0,1
0.0277777777777778,1
0.0555555555555556,1
0.0833333333333333,1
0.111111111111111,1
0.138888888888889,1
0.166666666666667,1
0.194444444444444,0.9999
0.222222222222222,0.9999
0.25,0.9999
0.277777777777778,0.9998
0.305555555555556,0.9997
0.333333333333333,0.9997
0.361111111111111,0.9996
0.388888888888889,0.9994
0.416666666666667,0.9993
0.444444444444444,0.9992
0.472222222222222,0.9991
0.5,0.9991
0.527777777777778,0.999
0.555555555555556,0.9989
0.583333333333333,0.9988
0.611111111111111,0.9986
0.638888888888889,0.9986
0.666666666666667,0.9986
0.694444444444444,0.9985
0.722222222222222,0.9985
0.75,0.9984
0.777777777777778,0.9984
0.805555555555556,0.9983
0.833333333333333,0.9977
0.861111111111111,0.9975
0.888888888888889,0.9973
0.916666666666667,0.9973
0.944444444444444,0.9973
0.972222222222222,0.9969
1,0.9957


==> data/datatool/vr_soa_set.tex <==
Instance,N,E,BASELINE_10,BASELINE_50,BASELINE,METAMIS_Cold,METAMIS_Warm,ILP,CHILS_Warm,CHILS_Cold,MaxWeight,MaxWeightCold,ilpWeightPerf,chilsWarmWeightPerf,baseWeightPerf,chilsColdWeightPerf,metamisColdWeightPerf,metamisWarmWeightPerf
CR-S-L-1,863368,331203970,5678316,5690529,5694508,5588489,5692891,5639292,5701015,5698608,5701015,5698608,0.989,1,0.9989,0.9996,0.9803,0.9986
CR-S-L-2,880974,342158741,5768571,5781233,5785140,5691892,5784034,5729194,5799458,5798470,5799458,5798470,0.988,1,0.9975,0.9998,0.9815,0.9973
CR-S-L-4,881910,344057350,5762528,5776186,5781519,5681336,5777081,5725525,5792758,5791447,5792758,5791447,0.988,1,0.9981,0.9998,0.9808,0.9973
CR-S-L-6,578244,219717582,3928270,3934574,3936944,3859513,3936137,3900370,3946157,3938946,3946157,3938946,0.988,1,0.9977,0.9982,0.978,0.9975
CR-S-L-7,270067,94109215,2015619,2016899,2017624,1989879,2019428,2006810,2022339,2021238,2022339,2021238,0.992,1,0.9977,0.9995,0.9839,0.9986
CR-T-C-1,602472,194753152,4731538,4739822,4742508,4654419,4743040,4717754,4750570,4744119,4750570,4744119,0.993,1,0.9983,0.9986,0.9798,0.9984
CR-T-C-2,652497,215694927,4958256,4967381,4969512,4874346,4968952,4934488,4976613,4975069,4976613,4975069,0.992,1,0.9986,0.9997,0.9795,0.9985
CR-T-D-4,651861,220480534,4898598,4910257,4912984,4817281,4911646,4875268,4922752,4919079,4922752,4919079,0.99,1,0.998,0.9993,0.9786,0.9977
CR-T-D-6,381380,115082762,3018014,3023382,3024044,2970011,3024523,3009020,3029782,3027211,3029782,3027211,0.993,1,0.9981,0.9992,0.9803,0.9983
CR-T-D-7,163809,43028583,1459286,1459997,1460328,1440281,1460240,1453990,1460584,1461099,1461099,1461099,0.995,0.9996,0.9995,1,0.9858,0.9994
CW-S-L-1,411950,283860106,1656670,1659095,1660063,1634950,1660815,1645459,1662580,1660472,1662580,1660472,0.99,1,0.9985,0.9987,0.9834,0.9989
CW-S-L-2,443404,315569883,1731390,1735389,1737052,1708820,1738128,1713535,1739670,1738307,1739670,1738307,0.985,1,0.9985,0.9992,0.9823,0.9991
CW-S-L-4,430379,303042962,1745476,1749887,1751204,1725591,1753803,1730641,1756602,1754409,1756602,1754409,0.985,1,0.9969,0.9988,0.9823,0.9984
CW-S-L-6,267698,171132761,1173871,1174628,1175335,1158925,1177156,1162552,1176354,1177272,1177272,1177272,0.987,0.9992,0.9984,1,0.9844,0.9999
CW-S-L-7,127871,78459291,593293,594069,594312,587288,593891,588279,593807,594598,594598,594598,0.989,0.9987,0.9995,1,0.9877,0.9988
CW-T-C-1,266403,144634578,1333264,1335859,1336232,1317775,1338064,1325862,1340085,1338085,1340085,1338085,0.989,1,0.9971,0.9985,0.9834,0.9985
CW-T-C-2,194413,111098006,943129,944398,944902,931802,945886,935238,945913,946217,946217,946217,0.988,0.9997,0.9986,1,0.9848,0.9997
CW-T-D-4,83091,37881529,460700,460877,460955,457185,461056,459575,461108,460734,461108,460734,0.997,1,0.9997,0.9992,0.9915,0.9999
CW-T-D-6,83758,38781839,460776,461022,461088,457790,461312,459238,461101,461354,461354,461354,0.995,0.9995,0.9994,1,0.9923,0.9999
MR-D-03,21499,130508,1751485940,1752842811,1752894190,1754110286,1757227519,1757141345,1758429721,1758762733,1758762733,1758762733,0.999,0.9998,0.9967,1,0.9974,0.9991
MR-D-05,27621,236044,1779855131,1781712136,1781868583,1786342921,1787849777,1788812740,1789537256,1789601100,1789601100,1789601100,1,1,0.9957,1,0.9982,0.999
MR-D-FN,30467,296369,1790740953,1793222332,1794240970,1797573192,1799452160,1801983754,1800375890,1801499264,1801983754,1801983754,1,0.9991,0.9957,0.9997,0.9976,0.9986
MR-W-FN,15639,126800,5385797991,5385799979,5385799979,5358386615,5386842781,5386842780,5386842781,5385799979,5386842781,5386842780,1,1,0.9998,0.9998,0.9947,1
MT-D-01,979,3125,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,1,1,1,1,1,1
MT-D-200,10880,505359,286834310,287042596,287042596,287048909,287048081,287155108,287042596,287086442,287155108,287155108,1,0.9996,0.9996,0.9998,0.9996,0.9996
MT-D-FN,10880,604041,290775742,290866943,290866943,290866943,290771450,290866943,290771450,290866943,290866943,290866943,1,0.9997,1,1,1,0.9997
MT-W-01,1006,2411,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,1,1,1,1,1,1
MT-W-200,12320,515871,383952339,383964395,383974084,383961323,383985408,384056011,384052017,384052157,384056011,384056011,1,1,0.9998,1,0.9998,0.9998
MT-W-FN,12320,553895,390863744,390869891,390869891,390854593,390869891,390869890,390869891,390869891,390869891,390869891,1,1,1,1,1,1
MW-D-01,3988,13556,475180516,475180516,475180516,476334711,475987082,476298607,476120423,476328138,476334711,476334711,1,0.9996,0.9976,1,1,0.9993
MW-D-20,20054,606318,522901741,523206860,523423307,525124575,525486034,526857183,526333489,526883302,526883302,526883302,1,0.999,0.9934,1,0.9967,0.9973
MW-D-40,33563,1879303,533054122,533629312,533671730,536520199,536735155,539036121,537485389,538302190,539036121,539036121,1,0.9971,0.99,0.9986,0.9953,0.9957
MW-D-FN,47504,4017196,540621713,541181146,541193604,541918916,543857187,545554192,544205239,544451893,545554192,545554192,1,0.9975,0.992,0.998,0.9933,0.9969
MW-W-01,3079,22664,1270305952,1270305952,1270305952,1270305952,1269344846,1270305952,1269344846,1270235200,1270305952,1270305952,1,0.9992,1,0.9999,1,0.9992
MW-W-05,10790,485261,1327478708,1327478708,1327478708,1328958047,1328958047,1326236043,1328958047,1328043785,1328958047,1328958047,0.998,1,0.9989,0.9993,1,1
MW-W-10,18023,1451813,1323128215,1340268013,1340268013,1342899725,1342915691,1280286209,1342915691,1342808634,1342915691,1342899725,0.953,1,0.998,0.9999,1,1
MW-W-FN,22316,2275623,1329149417,1331333002,1331333002,1350818543,1350818543,1235306258,1350818543,1350818543,1350818543,1350818543,0.914,1,0.9856,1,1,1


==> data/datatool/vr_soa_set10.tex <==
Instance,N,E,BASELINE10,BASELINE50,BASELINE,METAMIS_Cold,METAMIS_Warm,ILP,CHILS_Warm,CHILS_Cold,MaxWeight,MaxWeightCold,ilpWeightPerf,chilsWarmWeightPerf,baseWeightPerf,chilsColdWeightPerf,metamisColdWeightPerf,metamisWarmWeightPerf
CR-S-L-1,863368,331203970,5678316,5690529,5694508,5547038,5672398,2364648,5677207,5645288,5677207,5645288,0.4165,1,1.0002,0.9944,0.9771,0.9992
CR-S-L-2,880974,342158741,5768571,5781233,5785140,5652928,5763866,2356603,5767137,5737044,5767137,5737044,0.4086,1,1.0002,0.9948,0.9802,0.9994
CR-S-L-4,881910,344057350,5762528,5776186,5781519,5634886,5756016,2377801,5760039,5733355,5760039,5733355,0.4128,1,1.0004,0.9954,0.9783,0.9993
CR-S-L-6,578244,219717582,3928270,3934574,3936944,3833391,3926517,3876591,3932108,3912350,3932108,3912350,0.9859,1,0.999,0.995,0.9749,0.9986
CR-S-L-7,270067,94109215,2015619,2016899,2017624,1977161,2014584,2000653,2016526,2010023,2016526,2010023,0.9921,1,0.9996,0.9968,0.9805,0.999
CR-T-C-1,602472,194753152,4731538,4739822,4742508,4617204,4730533,4700095,4733127,4713081,4733127,4713081,0.993,1,0.9997,0.9958,0.9755,0.9995
CR-T-C-2,652497,215694927,4958256,4967381,4969512,4834040,4954613,4905655,4955534,4936378,4955534,4936378,0.9899,1,1.0005,0.9961,0.9755,0.9998
CR-T-D-4,651861,220480534,4898598,4910257,4912984,4778868,4898377,4825967,4900379,4882515,4900379,4882515,0.9848,1,0.9996,0.9964,0.9752,0.9996
CR-T-D-6,381380,115082762,3018014,3023382,3024044,2945721,3017902,3000784,3020589,3009362,3020589,3009362,0.9934,1,0.9991,0.9963,0.9752,0.9991
CR-T-D-7,163809,43028583,1459286,1459997,1460328,1431915,1458949,1452069,1459719,1457584,1459719,1457584,0.9948,1,0.9997,0.9985,0.981,0.9995
CW-S-L-1,411950,283860106,1656670,1659095,1660063,1623280,1656404,1632880,1656882,1649442,1656882,1649442,0.9855,1,0.9999,0.9955,0.9797,0.9997
CW-S-L-2,443404,315569883,1731390,1735389,1737052,1695131,1731077,1697231,1730571,1721277,1731077,1721277,0.9804,0.9997,1.0002,0.9943,0.9792,1
CW-S-L-4,430379,303042962,1745476,1749887,1751204,1712553,1748029,1715713,1748143,1737327,1748143,1737327,0.9814,1,0.9985,0.9938,0.9796,0.9999
CW-S-L-6,267698,171132761,1173871,1174628,1175335,1150229,1174005,1158222,1173885,1171256,1174005,1171256,0.9866,0.9999,0.9999,0.9977,0.9797,1
CW-S-L-7,127871,78459291,593293,594069,594312,582925,593045,586561,593308,592368,593308,592368,0.9886,1,1,0.9984,0.9825,0.9996
CW-T-C-1,266403,144634578,1333264,1335859,1336232,1310223,1334884,1317802,1334324,1328365,1334884,1328365,0.9872,0.9996,0.9988,0.9951,0.9815,1
CW-T-C-2,194413,111098006,943129,944398,944902,924664,944404,932639,944240,941498,944404,941498,0.9875,0.9998,0.9986,0.9969,0.9791,1
CW-T-D-4,83091,37881529,460700,460877,460955,454769,460643,458786,460756,459918,460756,459918,0.9957,1,0.9999,0.9982,0.987,0.9998
CW-T-D-6,83758,38781839,460776,461022,461088,455823,460982,458673,460878,460182,460982,460182,0.995,0.9998,0.9996,0.9983,0.9888,1
MR-D-03,21499,130508,1751485940,1752842811,1752894190,1753188475,1756186736,1757103978,1757110989,1756605513,1757110989,1757103978,1,1,0.9968,0.9997,0.9978,0.9995
MR-D-05,27621,236044,1779855131,1781712136,1781868583,1784519403,1787220357,1788491732,1787793221,1786854911,1788491732,1788491732,1,0.9996,0.9952,0.9991,0.9978,0.9993
MR-D-FN,30467,296369,1790740953,1793222332,1794240970,1795912642,1798215807,1801638038,1799200742,1797653553,1801638038,1801638038,1,0.9986,0.994,0.9978,0.9968,0.9981
MR-W-FN,15639,126800,5385797991,5385799979,5385799979,5357026363,5386842781,5386842780,5386842781,5385799979,5386842781,5386842780,1,1,0.9998,0.9998,0.9945,1
MT-D-01,979,3125,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,1,1,1,1,1,1
MT-D-200,10880,505359,286834310,287042596,287042596,286976422,287038328,287155108,286919240,287068605,287155108,287155108,1,0.9992,0.9989,0.9997,0.9994,0.9996
MT-D-FN,10880,604041,290775742,290866943,290866943,290866943,290771450,290800403,290761677,290866943,290866943,290866943,0.9998,0.9996,0.9997,1,1,0.9997
MT-W-01,1006,2411,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,1,1,1,1,1,1
MT-W-200,12320,515871,383952339,383964395,383974084,383818136,383971124,384056011,383933374,384052017,384056011,384056011,1,0.9997,0.9997,1,0.9994,0.9998
MT-W-FN,12320,553895,390863744,390869891,390869891,390688944,390828160,390869890,390830092,390863359,390869890,390869890,1,0.9999,1,1,0.9995,0.9999
MW-D-01,3988,13556,475180516,475180516,475180516,476099262,475886356,476098681,476040504,476313972,476313972,476313972,0.9995,0.9994,0.9976,1,0.9995,0.9991
MW-D-20,20054,606318,522901741,523206860,523423307,524255389,525052532,526383605,525331247,524946779,526383605,526383605,1,0.998,0.9934,0.9973,0.996,0.9975
MW-D-40,33563,1879303,533054122,533629312,533671730,533934442,535705687,538539768,535966879,535784778,538539768,538539768,1,0.9952,0.9898,0.9949,0.9914,0.9947
MW-D-FN,47504,4017196,540621713,541181146,541193604,539754400,543098071,544830719,543155166,541086426,544830719,544830719,1,0.9969,0.9923,0.9931,0.9907,0.9968
MW-W-01,3079,22664,1270305952,1270305952,1270305952,1270305952,1269314742,1270305952,1269344846,1270235200,1270305952,1270305952,1,0.9992,1,0.9999,1,0.9992
MW-W-05,10790,485261,1327478708,1327478708,1327478708,1328958047,1328958047,1317677026,1328958047,1328043785,1328958047,1328958047,0.9915,1,0.9989,0.9993,1,1
MW-W-10,18023,1451813,1323128215,1340268013,1340268013,1340878388,1342915691,1269692430,1342915691,1342402698,1342915691,1342402698,0.9455,1,0.9853,0.9996,0.9985,1
MW-W-FN,22316,2275623,1329149417,1331333002,1331333002,1349369736,1350814699,1229655165,1350818543,1350597182,1350818543,1350597182,0.9103,1,0.984,0.9998,0.9989,1


==> data/datatool/vr_soa_set50.tex <==
Instance,N,E,BASELINE10,BASELINE50,BASELINE,METAMIS_Cold,METAMIS_Warm,ILP,CHILS_Warm,CHILS_Cold,MaxWeight,MaxWeightCold,ilpWeightPerf,chilsWarmWeightPerf,baseWeightPerf,chilsColdWeightPerf,metamisColdWeightPerf,metamisWarmWeightPerf
CR-S-L-1,863368,331203970,5678316,5690529,5694508,5575602,5686939,5628809,5698548,5690025,5698548,5690025,0.9878,1,0.9986,0.9985,0.9784,0.998
CR-S-L-2,880974,342158741,5768571,5781233,5785140,5680688,5780859,5715690,5796291,5788627,5796291,5788627,0.9861,1,0.9974,0.9987,0.9801,0.9973
CR-S-L-4,881910,344057350,5762528,5776186,5781519,5671369,5771410,5708506,5788315,5782871,5788315,5782871,0.9862,1,0.9979,0.9991,0.9798,0.9971
CR-S-L-6,578244,219717582,3928270,3934574,3936944,3851432,3933476,3896797,3944667,3934036,3944667,3934036,0.9879,1,0.9974,0.9973,0.9764,0.9972
CR-S-L-7,270067,94109215,2015619,2016899,2017624,1986354,2018371,2004726,2021444,2019790,2021444,2019790,0.9917,1,0.9978,0.9992,0.9826,0.9985
CR-T-C-1,602472,194753152,4731538,4739822,4742508,4644635,4739684,4714415,4748826,4738351,4748826,4738351,0.9928,1,0.9981,0.9978,0.9781,0.9981
CR-T-C-2,652497,215694927,4958256,4967381,4969512,4863054,4966121,4930475,4974325,4967010,4974325,4967010,0.9912,1,0.9986,0.9985,0.9776,0.9984
CR-T-D-4,651861,220480534,4898598,4910257,4912984,4808490,4908285,4866470,4919890,4911446,4919890,4911446,0.9891,1,0.998,0.9983,0.9774,0.9976
CR-T-D-6,381380,115082762,3018014,3023382,3024044,2964007,3022448,3007188,3028351,3023310,3028351,3023310,0.993,1,0.9984,0.9983,0.9788,0.9981
CR-T-D-7,163809,43028583,1459286,1459997,1460328,1438896,1459958,1453380,1460468,1460794,1460794,1460794,0.9949,0.9998,0.9995,1,0.985,0.9994
CW-S-L-1,411950,283860106,1656670,1659095,1660063,1630417,1660475,1643209,1662168,1658769,1662168,1658769,0.9886,1,0.9982,0.998,0.9809,0.999
CW-S-L-2,443404,315569883,1731390,1735389,1737052,1704424,1735964,1711131,1738643,1736396,1738643,1736396,0.9842,1,0.9981,0.9987,0.9803,0.9985
CW-S-L-4,430379,303042962,1745476,1749887,1751204,1722542,1752354,1726645,1754918,1752181,1754918,1752181,0.9839,1,0.9971,0.9984,0.9816,0.9985
CW-S-L-6,267698,171132761,1173871,1174628,1175335,1156916,1175931,1161991,1175744,1175815,1175931,1175815,0.9881,0.9998,0.9989,0.9999,0.9838,1
CW-S-L-7,127871,78459291,593293,594069,594312,585929,593744,587974,593700,594511,594511,594511,0.989,0.9986,0.9993,1,0.9856,0.9987
CW-T-C-1,266403,144634578,1333264,1335859,1336232,1315122,1336953,1325112,1339364,1336441,1339364,1336441,0.9894,1,0.9974,0.9978,0.9819,0.9982
CW-T-C-2,194413,111098006,943129,944398,944902,929626,945748,933931,945700,944913,945748,944913,0.9875,0.9999,0.9986,0.9991,0.983,1
CW-T-D-4,83091,37881529,460700,460877,460955,456565,461027,459518,461108,460673,461108,460673,0.9966,1,0.9995,0.9991,0.9901,0.9998
CW-T-D-6,83758,38781839,460776,461022,461088,457382,461223,459073,461101,461297,461297,461297,0.9952,0.9996,0.9994,1,0.9915,0.9998
MR-D-03,21499,130508,1751485940,1752842811,1752894190,1753968167,1756989875,1757131533,1758218842,1758372635,1758372635,1758372635,0.9993,0.9999,0.9969,1,0.9975,0.9992
MR-D-05,27621,236044,1779855131,1781712136,1781868583,1785664042,1787666207,1788775706,1789482167,1789329743,1789482167,1789329743,0.9996,1,0.9957,0.9999,0.9979,0.999
MR-D-FN,30467,296369,1790740953,1793222332,1794240970,1797284091,1798926794,1801847126,1800197267,1800655663,1801847126,1801847126,1,0.9991,0.9952,0.9993,0.9975,0.9984
MR-W-FN,15639,126800,5385797991,5385799979,5385799979,5358386615,5386842781,5386842780,5386842781,5385799979,5386842781,5386842780,1,1,0.9998,0.9998,0.9947,1
MT-D-01,979,3125,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,1,1,1,1,1,1
MT-D-200,10880,505359,286834310,287042596,287042596,287048909,287048081,287155108,287039010,287086442,287155108,287155108,1,0.9996,0.9996,0.9998,0.9996,0.9996
MT-D-FN,10880,604041,290775742,290866943,290866943,290866943,290771450,290800403,290771450,290866943,290866943,290866943,0.9998,0.9997,1,1,1,0.9997
MT-W-01,1006,2411,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,1,1,1,1,1,1
MT-W-200,12320,515871,383952339,383964395,383974084,383961099,383985408,384056011,383986483,384052157,384056011,384056011,1,0.9998,0.9998,1,0.9998,0.9998
MT-W-FN,12320,553895,390863744,390869891,390869891,390830057,390869891,390869890,390836240,390869891,390869891,390869891,1,0.9999,1,1,0.9999,1
MW-D-01,3988,13556,475180516,475180516,475180516,476164209,475987082,476298607,476120423,476313972,476313972,476313972,1,0.9996,0.9976,1,0.9997,0.9993
MW-D-20,20054,606318,522901741,523206860,523423307,525036493,525402318,526857183,526150894,526306065,526857183,526857183,1,0.9987,0.9931,0.999,0.9965,0.9972
MW-D-40,33563,1879303,533054122,533629312,533671730,535707479,536210247,538925612,537197318,537898539,538925612,538925612,1,0.9968,0.9902,0.9981,0.994,0.995
MW-D-FN,47504,4017196,540621713,541181146,541193604,541372345,543622238,545439620,543800612,543526957,545439620,545439620,1,0.997,0.9922,0.9965,0.9925,0.9967
MW-W-01,3079,22664,1270305952,1270305952,1270305952,1270305952,1269344846,1270305952,1269344846,1270235200,1270305952,1270305952,1,0.9992,1,0.9999,1,0.9992
MW-W-05,10790,485261,1327478708,1327478708,1327478708,1328958047,1328958047,1326235998,1328958047,1328043785,1328958047,1328958047,0.998,1,0.9989,0.9993,1,1
MW-W-10,18023,1451813,1323128215,1340268013,1340268013,1342899725,1342915691,1280223475,1342915691,1342779166,1342915691,1342899725,0.9533,1,0.998,0.9999,1,1
MW-W-FN,22316,2275623,1329149417,1331333002,1331333002,1350818543,1350814699,1231751177,1350818543,1350818543,1350818543,1350818543,0.9119,1,0.9856,1,1,1


==> data/datatool/vr_soa_set_best.tex <==
Instance,N,E,BASELINE_10,BASELINE_50,BASELINE,METAMIS_Cold,METAMIS_Warm,ILP,CHILS_Warm,CHILS_Cold,CHILS_Par,CHILS_Reduced,MaxWeight,MaxWeightCold,ilpWeightPerf,chilsParWeightPerf,chilsWarmWeightPerf,baseWeightPerf,chilsColdWeightPerf,metamisColdWeightPerf,metamisWarmWeightPerf,chilsRedWeightPerf
CR-S-L-1,863368,331203970,5678316,5690529,5694508,5588489,5692891,5639292,5701015,5698608,5718230,5610201,5718230,5698608,0.986,1,0.997,0.9959,0.9966,0.9773,0.9956,0.9811
CR-S-L-2,880974,342158741,5768571,5781233,5785140,5691892,5784034,5729194,5799458,5798470,5813362,5715463,5813362,5798470,0.986,1,0.9976,0.9951,0.9974,0.9791,0.995,0.9832
CR-S-L-4,881910,344057350,5762528,5776186,5781519,5681336,5777081,5725525,5792758,5791447,5806975,5698425,5806975,5791447,0.986,1,0.9976,0.9956,0.9973,0.9784,0.9949,0.9813
CR-S-L-6,578244,219717582,3928270,3934574,3936944,3859513,3936137,3900370,3946157,3938946,3952205,3890733,3952205,3938946,0.987,1,0.9985,0.9961,0.9966,0.9765,0.9959,0.9844
CR-S-L-7,270067,94109215,2015619,2016899,2017624,1989879,2019428,2006810,2022339,2021238,2025681,2006857,2025681,2021238,0.991,1,0.9984,0.996,0.9978,0.9823,0.9969,0.9907
CR-T-C-1,602472,194753152,4731538,4739822,4742508,4654419,4743040,4717754,4750570,4744119,4760428,4702548,4760428,4744119,0.991,1,0.9979,0.9962,0.9966,0.9777,0.9963,0.9878
CR-T-C-2,652497,215694927,4958256,4967381,4969512,4874346,4968952,4934488,4976613,4975069,4987562,4918257,4987562,4975069,0.989,1,0.9978,0.9964,0.9975,0.9773,0.9963,0.9861
CR-T-D-4,651861,220480534,4898598,4910257,4912984,4817281,4911646,4875268,4922752,4919079,4932826,4864858,4932826,4919079,0.988,1,0.998,0.996,0.9972,0.9766,0.9957,0.9862
CR-T-D-6,381380,115082762,3018014,3023382,3024044,2970011,3024523,3009020,3029782,3027211,3033189,2999231,3033189,3027211,0.992,1,0.9989,0.997,0.998,0.9792,0.9971,0.9888
CR-T-D-7,163809,43028583,1459286,1459997,1460328,1440281,1460240,1453990,1460584,1461099,1462239,1451070,1462239,1461099,0.994,1,0.9989,0.9987,0.9992,0.985,0.9986,0.9924
CW-S-L-1,411950,283860106,1656670,1659095,1660063,1634950,1660815,1645459,1662580,1660472,1663763,1646548,1663763,1660472,0.989,1,0.9993,0.9978,0.998,0.9827,0.9982,0.9897
CW-S-L-2,443404,315569883,1731390,1735389,1737052,1708820,1738128,1713535,1739670,1738307,1743532,1723914,1743532,1738307,0.983,1,0.9978,0.9963,0.997,0.9801,0.9969,0.9887
CW-S-L-4,430379,303042962,1745476,1749887,1751204,1725591,1753803,1730641,1756602,1754409,1759452,1735633,1759452,1754409,0.984,1,0.9984,0.9953,0.9971,0.9808,0.9968,0.9865
CW-S-L-6,267698,171132761,1173871,1174628,1175335,1158925,1177156,1162552,1176354,1177272,1178467,1166774,1178467,1177272,0.986,1,0.9982,0.9973,0.999,0.9834,0.9989,0.9901
CW-S-L-7,127871,78459291,593293,594069,594312,587288,593891,588279,593807,594598,594757,590834,594757,594598,0.989,1,0.9984,0.9993,0.9997,0.9874,0.9985,0.9934
CW-T-C-1,266403,144634578,1333264,1335859,1336232,1317775,1338064,1325862,1340085,1338085,1341888,1323170,1341888,1338085,0.988,1,0.9987,0.9958,0.9972,0.982,0.9972,0.9861
CW-T-C-2,194413,111098006,943129,944398,944902,931802,945886,935238,945913,946217,947644,935907,947644,946217,0.987,1,0.9982,0.9971,0.9985,0.9833,0.9981,0.9876
CW-T-D-4,83091,37881529,460700,460877,460955,457185,461056,459575,461108,460734,461475,459543,461475,460734,0.996,1,0.9992,0.9989,0.9984,0.9907,0.9991,0.9958
CW-T-D-6,83758,38781839,460776,461022,461088,457790,461312,459238,461101,461354,461709,460227,461709,461354,0.995,1,0.9987,0.9987,0.9992,0.9915,0.9991,0.9968
MR-D-03,21499,130508,1751485940,1752842811,1752894190,1754110286,1757227519,1757141345,1758429721,1758762733,1759255435,1758775738,1759255435,1758762733,0.999,1,0.9995,0.9964,0.9997,0.9971,0.9988,0.9997
MR-D-05,27621,236044,1779855131,1781712136,1781868583,1786342921,1787849777,1788812740,1789537256,1789601100,1790776639,1789944187,1790776639,1789601100,0.999,1,0.9993,0.995,0.9993,0.9975,0.9984,0.9995
MR-D-FN,30467,296369,1790740953,1793222332,1794240970,1797573192,1799452160,1801983754,1800375890,1801499264,1802925854,1801727328,1802925854,1801983754,0.999,1,0.9986,0.9952,0.9992,0.997,0.9981,0.9993
MR-W-FN,15639,126800,5385797991,5385799979,5385799979,5358386615,5386842781,5386842780,5386842781,5385799979,5386842781,5386842781,5386842781,5386842780,1,1,1,0.9998,0.9998,0.9947,1,1
MT-D-01,979,3125,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,238166485,1,1,1,1,1,1,1,1
MT-D-200,10880,505359,286834310,287042596,287042596,287048909,287048081,287155108,287042596,287086442,287086442,287086442,287155108,287155108,1,0.9998,0.9996,0.9996,0.9998,0.9996,0.9996,0.9998
MT-D-FN,10880,604041,290775742,290866943,290866943,290866943,290771450,290866943,290771450,290866943,290866943,290866943,290866943,290866943,1,1,0.9997,1,1,1,0.9997,1
MT-W-01,1006,2411,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,312121568,1,1,1,1,1,1,1,1
MT-W-200,12320,515871,383952339,383964395,383974084,383961323,383985408,384056011,384052017,384052157,384056012,384052157,384056012,384056011,1,1,1,0.9998,1,0.9998,0.9998,1
MT-W-FN,12320,553895,390863744,390869891,390869891,390854593,390869891,390869890,390869891,390869891,390869891,390869891,390869891,390869891,1,1,1,1,1,1,1,1
MW-D-01,3988,13556,475180516,475180516,475180516,476334711,475987082,476298607,476120423,476328138,476360408,476440656,476440656,476334711,1,0.9998,0.9993,0.9974,0.9998,0.9998,0.999,1
MW-D-20,20054,606318,522901741,523206860,523423307,525124575,525486034,526857183,526333489,526883302,527498481,526648329,527498481,526883302,0.999,1,0.9978,0.9923,0.9988,0.9955,0.9962,0.9984
MW-D-40,33563,1879303,533054122,533629312,533671730,536520199,536735155,539036121,537485389,538302190,538596069,538409586,539036121,539036121,1,0.9992,0.9971,0.99,0.9986,0.9953,0.9957,0.9988
MW-D-FN,47504,4017196,540621713,541181146,541193604,541918916,543857187,545554192,544205239,544451893,545711017,544246489,545711017,545554192,1,1,0.9972,0.9917,0.9977,0.9931,0.9966,0.9973
MW-W-01,3079,22664,1270305952,1270305952,1270305952,1270305952,1269344846,1270305952,1269344846,1270235200,1270305952,1270305952,1270305952,1270305952,1,1,0.9992,1,0.9999,1,0.9992,1
MW-W-05,10790,485261,1327478708,1327478708,1327478708,1328958047,1328958047,1326236043,1328958047,1328043785,1328958047,1328043785,1328958047,1328958047,0.998,1,1,0.9989,0.9993,1,1,0.9993
MW-W-10,18023,1451813,1323128215,1340268013,1340268013,1342899725,1342915691,1280286209,1342915691,1342808634,1342915691,1342809954,1342915691,1342899725,0.953,1,1,0.998,0.9999,1,1,0.9999
MW-W-FN,22316,2275623,1329149417,1331333002,1331333002,1350818543,1350818543,1235306258,1350818543,1350818543,1350818543,1350818543,1350818543,1350818543,0.914,1,1,0.9856,1,1,1,1


==> tables/soa_vr.tex <==
\npthousandsep{\,}

\setlength{\tabcolsep}{4pt} 
\begin{landscape}
    \begin{longtable}{lrrrrrrrrrrr}
\caption{Results for vehicle routing instances by Dong \etal~\cite{dong2021new}. The results for \metamis{} were taken from the paper by Dong \etal~\cite{metamis} since the code is not publicly available. Note that the authors of \metamis{} used the best out of four runs, while the results for \baseline{}, \pils{}, and \ilp{} were only run once. All the results show the best solution found after one hour.}\label{tab:vr_results}\\

& \multicolumn{4}{c}{\bfseries Cold Start} && \multicolumn{2}{c}{\bfseries Warm Start} && \multicolumn{1}{c}{\bfseries Reduced} && \multicolumn{1}{c}{\bfseries Parallel} \\
\cmidrule{2-5} \cmidrule{7-8} \cmidrule{10-10} \cmidrule{12-12}%
\endfirsthead

\multicolumn{12}{c}%
{{\bfseries Table \thetable\ continued from previous page.}} \\[2em]

& \multicolumn{4}{c}{\bfseries Cold Start} && \multicolumn{2}{c}{\bfseries Warm Start} && \multicolumn{1}{c}{\bfseries Reduced} && \multicolumn{1}{c}{\bfseries Parallel} \\
\cmidrule{2-5} \cmidrule{7-8} \cmidrule{10-10} \cmidrule{12-12}
\bfseries Instance &
\multicolumn{1}{c}{\metamis} &
\multicolumn{1}{c}{\ilp} &
\multicolumn{1}{c}{\baseline} &
\multicolumn{1}{c}{\pils} && 
\multicolumn{1}{c}{\metamis} &
\multicolumn{1}{c}{\pils} && 
\multicolumn{1}{c}{\pils} && 
\multicolumn{1}{c}{\pils} \\
\cmidrule{2-5} \cmidrule{7-8} \cmidrule{10-10} \cmidrule{12-12}%
\endhead

\midrule \multicolumn{12}{r}{\textit{Continued on next page}} \\
\multicolumn{12}{r}{\vspace{1.cm}} %
\endfoot

\endlastfoot

\bfseries Instance &
\multicolumn{1}{c}{\metamis} &
\multicolumn{1}{c}{\ilp} &
\multicolumn{1}{c}{\baseline} &
\multicolumn{1}{c}{\pils} && 
\multicolumn{1}{c}{\metamis} &
\multicolumn{1}{c}{\pils} && 
\multicolumn{1}{c}{\pils} && 
\multicolumn{1}{c}{\pils} \\
\cmidrule{2-5}\cmidrule{7-8}\cmidrule{10-10}\cmidrule{12-12}%

\input{tables/results.tex}
\end{longtable}
\end{landscape}
\DTLgdeletedb{DATA}


